Producers Equilibria and Dynamics in Engagement-Driven Recommender Systems

Online platforms such as YouTube, Instagram heavily rely on recommender systems to decide what content to present to users. Producers, in turn, often create content that is likely to be recommended to users and have users engage with it. To do so, producers try to align their content with the preferences of their targeted user base. In this work, we explore the equilibrium behavior of producers who are interested in maximizing user engagement. We study two variants of the content-serving rule for the platform's recommender system, and provide a structural characterization of producer behavior at equilibrium: namely, each producer chooses to focus on a single embedded feature. We further show that specialization, defined as different producers optimizing for distinct types of content, naturally emerges from the competition among producers trying to maximize user engagement. We provide a heuristic for computing equilibria of our engagement game, and evaluate it experimentally. We highlight i) the performance and convergence of our heuristic, ii) the degree of producer specialization, and iii) the impact of the content-serving rule on producer and user utilities at equilibrium and provide guidance on how to set the content-serving rule.

==> app_additional_data.tex <==
We consider two other real datasets: Amazon Music ratings \cite{amazon-ratings} and Rent the Runway clothing ratings \cite{rentrunway}. For the Amazon Music ratings we use the ratings only \code{Digital\_Music.csv} from \url{https://nijianmo.github.io/amazon/index.html}, this dataset has $\sim$ 1.5 million ratings, $840k$ unique users and $450k$ unique items. For Rent the Runway we use  \url{https://cseweb.ucsd.edu/~jmcauley/datasets.html#clothing_fit}, this dataset has $\sim 190k$ ratings, $100k$ unique users and $5.8k$ unique items. 

==> app_convtable.tex <==
We consider a grid of $5$ random seeds, $12$ different number of producers $(2, 5, 10, 20, 30 \ldots, 100)$, $4$ different dimensions for the embeddings $(5, 10, 15, 20)$. We observe that on each of these $240$ instances of (seeds $\times$ producers $\times$ dimensions), the softmax serving rule with temperatures $\tau \in \{100, 10, 1, 0.1\}$ \emph{always} converges to a unique NE on all the datasets.  With softmax temperature $\tau=0.01$ (near-greedy) serving, Algorithm \ref{alg:bestrep_dynamics} still converges to a unique NE in a large number of instances. The linear-proportional serving also converges to a unique NE almost always.
\begin{table}[H]
\begin{tabular}{|l|r|r|r|r|r|r|}
\hline
Dataset           & \multicolumn{1}{l|}{Linear serving} & \multicolumn{1}{l|}{$\tau=100$} & \multicolumn{1}{l|}{$\tau=10$} & \multicolumn{1}{l|}{$\tau=1$} & \multicolumn{1}{l|}{$\tau=0.1$} & \multicolumn{1}{l|}{$\tau=0.01$} \\ \hline
Synthetic uniform & \textbf{239}                                 & 240                           & 240                          & 240                         & 240                           & \textbf{232}                            \\ \hline
Synthetic skewed  & 240                                 & 240                           & 240                          & 240                         & 240                           & \textbf{240}                            \\ \hline
Movielens-100k    & 240                                 & 240                           & 240                          & 240                         & 240                           & \textbf{233}                            \\ \hline
AmazonMusic       & 240                                 & 240                           & 240                          & 240                         & 240                           & \textbf{236}                            \\ \hline
RentTheRunway     & 240                                 & 240                           & 240                          & 240                         & 240                           & \textbf{237}                            \\ \hline
\end{tabular}
\captionof{table}{Number of instances in which Algorithm \ref{alg:bestrep_dynamics} run on the engagement game with various serving rules converges to a Nash equilibrium \label{table:appconv_table}}
\end{table}

==> app_experiments_utiltables.tex <==
In each of the experiments for the $3$ datasets: Uniform, MovieLens-100k, Skewed we considered $400$ instances of (seed, producers, dimension)\footnote{values provided in \code{README} of the supplementary}: $10$ random seeds, $10$ different number of producers($n = 10 \ldots 100$) and $4$ different dimensions($d = 5, 10, 15, 20$) of the embeddings. We then noted the user and producer utilities at the Nash equilibrium. In each of the experiments across all instances the linear-proportional content serving rule has greater than or equal utility compared to the softmax serving rule. Here, in Tables \ref{tab:uniform-dataset-utils}, \ref{tab:movielens-dataset-utils} and \ref{tab:skewed-dataset-utils} we present the utilities for each (dimension $d$, number of producers $n$) averaged across the $10$ random seeds.


\begin{table}[!h]
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{|ll|ll|ll|ll|ll|}
\hline
d &
  n &
  \begin{tabular}[c]{@{}l@{}}Mean \\ producer \\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Mean \\ producer\\ utility \\ (softmax)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ producer\\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ producer\\ utility \\ (softmax)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Mean \\ user\\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Mean \\ user\\ utility \\ (softmax)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ user\\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ user\\ utility \\ (softmax)\end{tabular} \\ \hline
5  & 10  & 333.50 & 228.70 & 326.80 & 227.00 & 0.334 & 0.229 & 0.201 & 0.177 \\
5  & 20  & 166.70 & 114.40 & 163.50 & 113.90 & 0.334 & 0.229 & 0.201 & 0.181 \\
5  & 30  & 111.10 & 76.27  & 109.40 & 76.04  & 0.333 & 0.229 & 0.201 & 0.184 \\
5  & 40  & 83.36  & 57.21  & 82.37  & 57.10  & 0.334 & 0.229 & 0.201 & 0.185 \\
5  & 50  & 66.69  & 45.77  & 65.98  & 45.68  & 0.334 & 0.229 & 0.201 & 0.185 \\
5  & 60  & 55.58  & 38.14  & 55.05  & 38.08  & 0.334 & 0.229 & 0.201 & 0.186 \\
5  & 70  & 47.64  & 32.69  & 47.25  & 32.65  & 0.334 & 0.229 & 0.201 & 0.185 \\
5  & 80  & 41.68  & 28.60  & 41.39  & 28.57  & 0.334 & 0.229 & 0.201 & 0.185 \\
5  & 90  & 37.05  & 25.43  & 36.83  & 25.40  & 0.334 & 0.229 & 0.201 & 0.185 \\
5  & 100 & 33.35  & 22.88  & 33.17  & 22.86  & 0.334 & 0.229 & 0.201 & 0.185 \\ \hline
10 & 10  & 181.90 & 108.70 & 177.30 & 108.20 & 0.182 & 0.109 & 0.106 & 0.025 \\
10 & 20  & 90.95  & 54.40  & 88.63  & 54.28  & 0.182 & 0.109 & 0.106 & 0.032 \\
10 & 30  & 60.63  & 36.27  & 59.28  & 36.21  & 0.182 & 0.109 & 0.106 & 0.032 \\
10 & 40  & 45.47  & 27.20  & 44.61  & 27.17  & 0.182 & 0.109 & 0.106 & 0.032 \\
10 & 50  & 36.38  & 21.77  & 35.84  & 21.74  & 0.182 & 0.109 & 0.106 & 0.034 \\
10 & 60  & 30.32  & 18.14  & 29.95  & 18.12  & 0.182 & 0.109 & 0.106 & 0.032 \\
10 & 70  & 25.99  & 15.55  & 25.72  & 15.53  & 0.182 & 0.109 & 0.105 & 0.033 \\
10 & 80  & 22.74  & 13.60  & 22.54  & 13.59  & 0.182 & 0.109 & 0.105 & 0.033 \\
10 & 90  & 20.21  & 12.09  & 20.05  & 12.09  & 0.182 & 0.109 & 0.106 & 0.033 \\
10 & 100 & 18.19  & 10.88  & 18.06  & 10.88  & 0.182 & 0.109 & 0.106 & 0.033 \\ \hline
15 & 10  & 122.00 & 71.03  & 119.60 & 70.85  & 0.122 & 0.071 & 0.032 & 0.009 \\
15 & 20  & 62.31  & 35.53  & 59.92  & 35.48  & 0.125 & 0.071 & 0.075 & 0.010 \\
15 & 30  & 41.65  & 23.69  & 40.71  & 23.66  & 0.125 & 0.071 & 0.075 & 0.010 \\
15 & 40  & 31.24  & 17.76  & 30.62  & 17.75  & 0.125 & 0.071 & 0.075 & 0.010 \\
15 & 50  & 25.00  & 14.21  & 24.63  & 14.20  & 0.125 & 0.071 & 0.075 & 0.011 \\
15 & 60  & 20.84  & 11.84  & 20.56  & 11.84  & 0.125 & 0.071 & 0.075 & 0.010 \\
15 & 70  & 17.86  & 10.15  & 17.67  & 10.15  & 0.125 & 0.071 & 0.075 & 0.010 \\
15 & 80  & 15.63  & 8.88   & 15.47  & 8.88   & 0.125 & 0.071 & 0.076 & 0.010 \\
15 & 90  & 13.90  & 7.90   & 13.77  & 7.89   & 0.125 & 0.071 & 0.075 & 0.010 \\
15 & 100 & 12.51  & 7.11   & 12.40  & 7.10   & 0.125 & 0.071 & 0.075 & 0.010 \\ \hline
20 & 10  & 91.77  & 52.66  & 90.38  & 52.54  & 0.092 & 0.053 & 0.020 & 0.006 \\
20 & 20  & 47.60  & 26.34  & 45.90  & 26.31  & 0.095 & 0.053 & 0.056 & 0.006 \\
20 & 30  & 31.69  & 17.56  & 30.88  & 17.55  & 0.095 & 0.053 & 0.058 & 0.006 \\
20 & 40  & 23.80  & 13.17  & 23.34  & 13.16  & 0.095 & 0.053 & 0.058 & 0.006 \\
20 & 50  & 19.04  & 10.54  & 18.73  & 10.53  & 0.095 & 0.053 & 0.058 & 0.006 \\
20 & 60  & 15.87  & 8.78   & 15.67  & 8.78   & 0.095 & 0.053 & 0.058 & 0.006 \\
20 & 70  & 13.61  & 7.53   & 13.43  & 7.52   & 0.095 & 0.053 & 0.058 & 0.006 \\
20 & 80  & 11.91  & 6.59   & 11.79  & 6.58   & 0.095 & 0.053 & 0.059 & 0.006 \\
20 & 90  & 10.58  & 5.85   & 10.48  & 5.85   & 0.095 & 0.053 & 0.059 & 0.006 \\
20 & 100 & 9.53   & 5.27   & 9.45   & 5.27   & 0.095 & 0.053 & 0.058 & 0.006 \\ \hline
\end{tabular}
}
\captionof{table}{\centering Producer and user utilities on the uniform dataset for both the content serving rules, averaged across 10 random seeds, the number of users is fixed to $10000$. \label{tab:uniform-dataset-utils}}
\end{table}

\begin{table}[!t]
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{|ll|ll|ll|ll|ll|}
\hline
d &
  n &
  \begin{tabular}[c]{@{}l@{}}Mean \\ producer \\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Mean \\ producer\\ utility \\ (softmax)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ producer\\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ producer\\ utility \\ (softmax)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Mean \\ user\\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Mean \\ user\\ utility \\ (softmax)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ user\\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ user\\ utility \\ (softmax)\end{tabular} \\ \hline
5  & 10  & 21.841 & 19.691 & 21.577 & 19.662 & 0.232 & 0.209 & 0.161 & 0.045 \\
5  & 20  & 10.926 & 9.845  & 10.857 & 9.840  & 0.232 & 0.209 & 0.163 & 0.045 \\
5  & 30  & 7.286  & 6.565  & 7.253  & 6.561  & 0.232 & 0.209 & 0.163 & 0.045 \\
5  & 40  & 5.466  & 4.923  & 5.447  & 4.922  & 0.232 & 0.209 & 0.167 & 0.045 \\
5  & 50  & 4.373  & 3.939  & 4.361  & 3.938  & 0.232 & 0.209 & 0.169 & 0.045 \\
5  & 60  & 3.644  & 3.282  & 3.636  & 3.282  & 0.232 & 0.209 & 0.170 & 0.045 \\
5  & 70  & 3.123  & 2.813  & 3.118  & 2.813  & 0.232 & 0.209 & 0.168 & 0.045 \\
5  & 80  & 2.733  & 2.462  & 2.729  & 2.461  & 0.232 & 0.209 & 0.170 & 0.045 \\
5  & 90  & 2.429  & 2.188  & 2.426  & 2.188  & 0.232 & 0.209 & 0.169 & 0.045 \\
5  & 100 & 2.187  & 1.969  & 2.184  & 1.969  & 0.232 & 0.209 & 0.169 & 0.045 \\ \hline
10 & 10  & 12.015 & 9.902  & 11.787 & 9.895  & 0.127 & 0.105 & 0.075 & 0.012 \\
10 & 20  & 6.013  & 4.951  & 5.951  & 4.949  & 0.128 & 0.105 & 0.085 & 0.011 \\
10 & 30  & 4.011  & 3.301  & 3.982  & 3.300  & 0.128 & 0.105 & 0.088 & 0.011 \\
10 & 40  & 3.009  & 2.476  & 2.992  & 2.475  & 0.128 & 0.105 & 0.089 & 0.011 \\
10 & 50  & 2.407  & 1.981  & 2.396  & 1.980  & 0.128 & 0.105 & 0.089 & 0.011 \\
10 & 60  & 2.006  & 1.650  & 1.998  & 1.650  & 0.128 & 0.105 & 0.090 & 0.011 \\
10 & 70  & 1.720  & 1.415  & 1.714  & 1.414  & 0.128 & 0.105 & 0.090 & 0.011 \\
10 & 80  & 1.505  & 1.238  & 1.500  & 1.238  & 0.128 & 0.105 & 0.090 & 0.011 \\
10 & 90  & 1.338  & 1.100  & 1.334  & 1.100  & 0.128 & 0.105 & 0.090 & 0.011 \\
10 & 100 & 1.204  & 0.990  & 1.201  & 0.990  & 0.128 & 0.105 & 0.090 & 0.011 \\ \hline
15 & 10  & 8.466  & 6.594  & 8.274  & 6.588  & 0.090 & 0.070 & 0.048 & 0.005 \\
15 & 20  & 4.248  & 3.297  & 4.186  & 3.296  & 0.090 & 0.070 & 0.056 & 0.005 \\
15 & 30  & 2.832  & 2.198  & 2.808  & 2.198  & 0.090 & 0.070 & 0.057 & 0.005 \\
15 & 40  & 2.126  & 1.649  & 2.110  & 1.648  & 0.090 & 0.070 & 0.059 & 0.005 \\
15 & 50  & 1.700  & 1.319  & 1.690  & 1.319  & 0.090 & 0.070 & 0.059 & 0.005 \\
15 & 60  & 1.417  & 1.099  & 1.409  & 1.099  & 0.090 & 0.070 & 0.058 & 0.005 \\
15 & 70  & 1.215  & 0.942  & 1.210  & 0.942  & 0.090 & 0.070 & 0.059 & 0.005 \\
15 & 80  & 1.063  & 0.824  & 1.060  & 0.824  & 0.090 & 0.070 & 0.059 & 0.005 \\
15 & 90  & 0.945  & 0.733  & 0.942  & 0.733  & 0.090 & 0.070 & 0.059 & 0.005 \\
15 & 100 & 0.850  & 0.659  & 0.847  & 0.659  & 0.090 & 0.070 & 0.059 & 0.005 \\ \hline
20 & 10  & 6.562  & 4.974  & 6.407  & 4.971  & 0.070 & 0.053 & 0.034 & 0.002 \\
20 & 20  & 3.298  & 2.487  & 3.251  & 2.486  & 0.070 & 0.053 & 0.041 & 0.002 \\
20 & 30  & 2.201  & 1.658  & 2.178  & 1.658  & 0.070 & 0.053 & 0.042 & 0.002 \\
20 & 40  & 1.651  & 1.243  & 1.638  & 1.243  & 0.070 & 0.053 & 0.042 & 0.002 \\
20 & 50  & 1.321  & 0.995  & 1.312  & 0.995  & 0.070 & 0.053 & 0.042 & 0.002 \\
20 & 60  & 1.101  & 0.829  & 1.095  & 0.829  & 0.070 & 0.053 & 0.043 & 0.002 \\
20 & 70  & 0.944  & 0.711  & 0.940  & 0.711  & 0.070 & 0.053 & 0.042 & 0.002 \\
20 & 80  & 0.826  & 0.621  & 0.822  & 0.621  & 0.070 & 0.053 & 0.043 & 0.002 \\
20 & 90  & 0.734  & 0.553  & 0.731  & 0.553  & 0.070 & 0.053 & 0.043 & 0.002 \\
20 & 100 & 0.661  & 0.497  & 0.659  & 0.497  & 0.070 & 0.053 & 0.042 & 0.002 \\ \hline
\end{tabular}
}
\captionof{table}{\centering Producer and user utilities on the MovieLens-100k dataset for both the content serving rules, averaged across 10 random seeds, the number of users is the full $943$ available in MovieLens-100k.\label{tab:movielens-dataset-utils}}
\end{table}

\begin{table}[]
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{|ll|ll|ll|ll|ll|}
\hline
d &
  n &
  \begin{tabular}[c]{@{}l@{}}Mean \\ producer \\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Mean \\ producer\\ utility \\ (softmax)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ producer\\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ producer\\ utility \\ (softmax)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Mean \\ user\\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Mean \\ user\\ utility \\ (softmax)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ user\\ utility \\ (linear)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Min \\ user\\ utility \\ (softmax)\end{tabular} \\ \hline
5  & 10  & 456.00 & 401.08 & 445.63 & 399.48 & 0.45600 & 0.40108 & 0.01174 & 0.00432 \\
5  & 20  & 229.46 & 200.41 & 227.28 & 200.12 & 0.45893 & 0.40082 & 0.01442 & 0.00421 \\
5  & 30  & 153.07 & 133.65 & 151.90 & 133.52 & 0.45920 & 0.40094 & 0.02056 & 0.00428 \\
5  & 40  & 114.88 & 100.26 & 114.17 & 100.20 & 0.45952 & 0.40105 & 0.02055 & 0.00436 \\
5  & 50  & 91.83  & 80.19  & 91.28  & 80.15  & 0.45916 & 0.40095 & 0.02040 & 0.00436 \\
5  & 60  & 76.58  & 66.83  & 76.25  & 66.80  & 0.45951 & 0.40096 & 0.02047 & 0.00429 \\
5  & 70  & 65.67  & 57.29  & 65.41  & 57.26  & 0.45966 & 0.40101 & 0.02059 & 0.00432 \\
5  & 80  & 57.46  & 50.13  & 57.26  & 50.11  & 0.45970 & 0.40103 & 0.02062 & 0.00434 \\
5  & 90  & 51.07  & 44.56  & 50.91  & 44.54  & 0.45964 & 0.40100 & 0.02050 & 0.00434 \\
5  & 100 & 45.98  & 40.10  & 45.84  & 40.09  & 0.45977 & 0.40103 & 0.02068 & 0.00436 \\ \hline
10 & 10  & 290.21 & 233.43 & 282.65 & 232.82 & 0.29021 & 0.23343 & 0.00742 & 0.00336 \\
10 & 20  & 145.68 & 116.84 & 143.20 & 116.62 & 0.29135 & 0.23368 & 0.00921 & 0.00343 \\
10 & 30  & 97.26  & 77.84  & 96.07  & 77.76  & 0.29178 & 0.23352 & 0.00975 & 0.00320 \\
10 & 40  & 73.00  & 58.39  & 72.48  & 58.36  & 0.29198 & 0.23356 & 0.01016 & 0.00332 \\
10 & 50  & 58.52  & 46.73  & 58.17  & 46.69  & 0.29259 & 0.23363 & 0.01362 & 0.00337 \\
10 & 60  & 48.77  & 38.94  & 48.49  & 38.92  & 0.29260 & 0.23364 & 0.01535 & 0.00341 \\
10 & 70  & 41.80  & 33.38  & 41.55  & 33.36  & 0.29257 & 0.23364 & 0.01532 & 0.00338 \\
10 & 80  & 36.58  & 29.21  & 36.35  & 29.20  & 0.29260 & 0.23365 & 0.01685 & 0.00340 \\
10 & 90  & 32.50  & 25.96  & 32.38  & 25.95  & 0.29253 & 0.23364 & 0.01523 & 0.00339 \\
10 & 100 & 29.27  & 23.36  & 29.14  & 23.35  & 0.29272 & 0.23363 & 0.01681 & 0.00340 \\ \hline
15 & 10  & 236.21 & 191.87 & 229.82 & 191.63 & 0.23621 & 0.19187 & 0.00688 & 0.00064 \\
15 & 20  & 118.68 & 95.95  & 117.21 & 95.85  & 0.23735 & 0.19189 & 0.00807 & 0.00062 \\
15 & 30  & 79.24  & 63.96  & 78.38  & 63.93  & 0.23772 & 0.19189 & 0.00955 & 0.00061 \\
15 & 40  & 59.42  & 47.96  & 58.99  & 47.95  & 0.23769 & 0.19185 & 0.00914 & 0.00061 \\
15 & 50  & 47.56  & 38.38  & 47.23  & 38.37  & 0.23779 & 0.19189 & 0.00933 & 0.00062 \\
15 & 60  & 39.65  & 31.98  & 39.42  & 31.98  & 0.23789 & 0.19189 & 0.01024 & 0.00062 \\
15 & 70  & 33.97  & 27.41  & 33.81  & 27.41  & 0.23782 & 0.19187 & 0.01026 & 0.00062 \\
15 & 80  & 29.74  & 23.98  & 29.60  & 23.98  & 0.23794 & 0.19187 & 0.01022 & 0.00061 \\
15 & 90  & 26.46  & 21.32  & 26.38  & 21.32  & 0.23814 & 0.19189 & 0.01043 & 0.00062 \\
15 & 100 & 23.81  & 19.19  & 23.74  & 19.19  & 0.23811 & 0.19188 & 0.01031 & 0.00062 \\ \hline
20 & 10  & 188.74 & 144.18 & 182.61 & 143.90 & 0.18874 & 0.14418 & 0.00636 & 0.00060 \\
20 & 20  & 95.23  & 72.06  & 93.48  & 72.00  & 0.19045 & 0.14413 & 0.01010 & 0.00090 \\
20 & 30  & 63.45  & 48.06  & 62.59  & 48.03  & 0.19035 & 0.14417 & 0.01084 & 0.00094 \\
20 & 40  & 47.56  & 36.05  & 47.14  & 36.03  & 0.19025 & 0.14418 & 0.01082 & 0.00095 \\
20 & 50  & 38.13  & 28.84  & 37.80  & 28.83  & 0.19063 & 0.14418 & 0.01082 & 0.00095 \\
20 & 60  & 31.75  & 24.03  & 31.54  & 24.02  & 0.19049 & 0.14416 & 0.01091 & 0.00095 \\
20 & 70  & 27.23  & 20.60  & 27.09  & 20.59  & 0.19063 & 0.14418 & 0.01211 & 0.00095 \\
20 & 80  & 23.83  & 18.02  & 23.72  & 18.02  & 0.19061 & 0.14418 & 0.01208 & 0.00095 \\
20 & 90  & 21.19  & 16.02  & 21.09  & 16.02  & 0.19073 & 0.14418 & 0.01261 & 0.00095 \\
20 & 100 & 19.07  & 14.42  & 18.99  & 14.42  & 0.19070 & 0.14416 & 0.01256 & 0.00095 \\ \hline
\end{tabular}}
\captionof{table}{\centering Producer and user utilities on the skewed dataset for both the content serving rules, averaged across 10 random seeds, the number of users is fixed to 10000. \label{tab:skewed-dataset-utils}}
\end{table}

==> experiments.tex <==
\subsection{Experimental setup} 

\paragraph{Synthetic Data} We generate two types of user distributions for our synthetic data: \begin{itemize}
    \item \emph{Uniform distribution:} we generate user embeddings $c$ uniformly at random over the probability simplex. Each feature is roughly equally represented in the data (up to randomness). We refer to the dataset as the \emph{uniform dataset}.
    \item \emph{Skewed-uniform distribution:} we generate user embeddings $c$ according to what we call a \emph{skewed-uniform} distribution. To do so, we randomly sample positive weights $w_1 \leq \ldots \leq w_d$ (we sample weights from the probability simplex then sort them). We then generate a uniformly distributed user embedding, but re-weight each feature $f$ by $w_f$ to obtain $c$. This creates a non-symmetric and skewed distribution where the total user weight in each feature is different across different features, and proportional to $w_f$ for feature $f$. We refer to the dataset as the \emph{skewed dataset}.
\end{itemize}
To be consistent with our modeling assumptions, we normalize user representations $c$ to have norm $1$. All synthetic experiments use $K = 10,000$ users, but we vary the values of the dimension $d$ and of the number of producers $n$. 

\kri{Mention Amznmusic and Rentrunway too}
\paragraph{Real Data} We use the MovieLens-100k dataset~\citep{movielens}. We use Non-negative matrix factorization (NMF) to generate user embeddings, relying on the implementation from the scikit-surprise package~\citep{scikit-surprise}. We note that the dataset is comprised of $943$ users, a significantly smaller number than the $10,000$ we use for synthetic data, leading to more variability in our experimental results. \comment{We vary the embedding dimension $d$ across our experiments.}


\subsection{Experimental results}

\paragraph{Convergence of best response dynamics in Algorithm~\ref{alg:bestrep_dynamics}} Our best-response dynamics converge to an equilibrium \emph{in the large majority of cases} in our experiments. We do so by considering a grid of $10$ random seeds \footnote{We do so to deal with the randomness in the draws of the synthetic data, and the randomness of Non-negative matrix factorization algorithm for the MovieLens-100k data}, $10$ different number of producers $(10, \ldots, 100)$ and $4$ different dimensions for the embeddings $(5, 10, 15, 20)$. We observe that on all of these $400$ instances of (seed, producers, dimension), the softmax serving rule \emph{always} converges to a unique NE on all the $3$ datasets: uniform, skewed, and MovieLens-100k. The linear-proportional serving converges to a unique NE a vast majority of time: we observe convergence in $399$, $400$, $398$ out of the $400$ instances for the uniform, skewed and MovieLens-100k datasets respectively. 

We are also interested in characterizing the rate at which the best response dynamics converge. In Figure~\ref{fig:num_iters_convergence}, we iterate over $4$ values for the dimension $d$ of the factorization $d \in ( 5, 10, 15, 20)$. We plot the average number (over 40 runs) of iterations until the best response dynamics converge to a NE. Figure~\eqref{fig:convergence_linear} plots the time to convergence under the linear-proportional content serving rule, while Figure~\eqref{fig:convergence_softmax} plots the time to convergence under the softmax content serving rule. Both figures provide standard error bars to show the variability of our results. We see a time to convergence that seems to evolve linearly in the number of producers, implying strong computational efficiency and scaling properties. This is a departure from the naive brute-force approach that must enumerate all best responses, which takes exponential time over the number of producers. We extend the results to the MovieLens-100k and the skewed dataset in Appendix~\ref{app:num_iters}, and see similar insights.

 \begin{figure}[!h]
 \vspace{-3mm}
\centering
\subfloat[Linear-proportional content serving]{
    \includegraphics[width=0.23\textwidth]{Figures/num_iters/num_iter_unif_linear.pdf}\label{fig:convergence_linear}
}
\subfloat[Softmax content serving]{
    \includegraphics[width=0.23\textwidth]{Figures/num_iters/num_iter_unif_softmax.pdf}\label{fig:convergence_softmax}
} 
\vspace{-1mm}
\caption{Number of iterations of the best-response dynamics of Algorithm~\ref{alg:bestrep_dynamics} until convergence to a NE on the uniform dataset}\label{fig:num_iters_convergence}
\vspace{-1mm}
\end{figure}

Based on the observations above, we conclude that Algorithm~\ref{alg:bestrep_dynamics} seems to be a reliable and computationally efficient heuristic to find pure Nash equilibria in engagement games.

\paragraph{Producer and User utilities at equilibrium} We also measure the following metrics at NE: the average producer utility, minimum producer utility, and the average user utility and minimum user utility. We define the utility of a user $c_k$ as their total engagement across all producers, i.e. $\sum_{j = 1}^n p_j(c_k,\vec{s}) \cdot c_k^\top s_j$. For each of the datasets across all instances, the linear-proportional content serving rule has utility greater than or equal to the softmax content-serving rule for all the above metrics, (tables provided in Appendix \ref{app:util_tables}). We believe this provides an argument in favour of using our linear-proportional content-serving rule as opposed to the softmax rule of ~\cite{hron2022modeling}, as it provides higher utilities to both sides of the recommender system. 

\kri{6 plots temp 100,10,1,0.1,0.01 ad linear, dim = 15, fix number of producer to 100}
\kri{Average producer and user utility for dimension = 15, varying number of producers, 2 each for each dataset}
\paragraph{Equilibrium results}  For each of the user and producer distributions figures (Figures~\ref{fig:uniform_n100} to~\ref{fig:skewed_n100_softmax}), we show a single representative instance of the problem.
We do not provide standard errors, as in this case we note that the user embedding is deterministic and empirically observe the NE we recover is unique, hence our results are completely deterministic on a given instance. The reason we do not average over a large number of instances is that we are interested in highlighting specialization properties that arise at the level of each instance, not in expectation. 

Averaging across several instances can hide lack of specialization, in the following manner: in each instance, only a few features are targeted by the producers, like in Figure~\ref{fig:movielens-100k-softmax} for example. However, these features change as the specific instance we look at change. In that case, when averaging over many instances, we may be under the impression that specialization occurs, when it does not. 

In Figure~\ref{fig:uniform_n100}, we compute the Nash equilibria of our engagement game on synthetic data with uniformly-distributed users under the linear-proportional rule. Because users are uniformly distributed, we note that the average weight on each feature is roughly (but not exactly) the same across each feature. We observe high levels of specializations where the producers are spread out across all features; i.e. producers, at equilibrium, diversify their content from each other. Producers do not spread exactly evenly across features, due to randomness making some features slightly better and some slightly worse than others, but we still observe a relatively even spread. In Figure~\ref{fig:movielens-100k-linear}, we replicate this experiment on the MovieLens-100k dataset. Note that the user embeddings are obtained via NMF, we tend to get that the user weight is spread similarly across each feature in the embedding, as has been observed in the experiments of~\citet{meena-ss,hron2022modeling}; however, this is only true in an average sense, and features can change significantly per user. In fact, the feature distribution using NMF behaves similarly to our synthetic uniform distribution. We note that the insights from Figure~\ref{fig:movielens-100k-linear} then end up similar to those of Figure~\ref{fig:uniform_n100}. The main difference can be attributed to the fact that the MovieLens dataset contains only $943$ users, and there is more variability in the distribution of user features than our synthetic data. This can lead some features to be ignored: at equal average user weight, producers may prefer more features that have less variability, as they more reliably target a larger subset of the user population.

\begin{figure}[!h]
\vspace{-2mm}
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[Embedding dimension \\ $d = 5$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/uniformsynth_linear_dim5_100prod.pdf}}
\hfill
\subfloat[Embedding dimension \\ $d = 10$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/uniformsynth_linear_dim10_100prod.pdf}}
\hfill
\subfloat[Embedding dimension $d = 15$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/uniformsynth_linear_dim15_100prod.pdf}
}
\hfill
\subfloat[Embedding dimension $d = 20$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/uniformsynth_linear_dim20_100prod.pdf}
}
\caption{Average user weight on each feature (blue, left bar) and fraction of producers going for each feature (red, right bar) for the linear-proportional serving rule; $n = 100$ producers. Uniform distribution of users.\label{fig:uniform_n100}}
\end{figure}

\begin{figure}[!h]
\vspace{-1mm}
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[Embedding dimension \\$d = 5$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/Movielens_linear_dim5_100prod.pdf}
}
\subfloat[Embedding dimension \\$d = 10$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/Movielens_linear_dim10_100prod.pdf}
}
\hfill
\subfloat[Embedding dimension $d = 15$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/Movielens_linear_dim15_100prod.pdf}
}
\hfill
\subfloat[Embedding dimension $d = 20$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/Movielens_linear_dim20_100prod.pdf}
}
\caption{Average user weight on each feature (in blue) and fraction of producers going for each feature (in red) for the linear-proportional content serving rule with $n=100$ producers. User embeddings obtained from NMF on MovieLens-100k.\label{fig:movielens-100k-linear}}
\vspace{-5mm}
\end{figure}




In Figure~\ref{fig:uniformsoftmax_n100}, we consider users that are uniformly distributed, but the content-serving rule is now the softmax rule. We observe that few features are represented and that there is less content specialization. This is unsurprising, as the softmax function behaves closer to a maximum than our linear-proportional rule; for a given user $k$, the probability of showing content to that user (and hence the producer utility) goes disproportionally to the producers with the best fit to $k$'s preferences $c_k$. This strengthens producers' incentives to focus on the most rewarding features, i.e. that align as well as possible with as many users as possible. Even little variability across the distributions of different features can still lead to largely different investments in these features by different producers. Figure~\ref{fig:movielens-100k-softmax} replicates our experiments on the Movielens-100k dataset instead of our synthetic data, and exhibits similar insights.


\begin{figure}[!h]
\vspace{-1mm}
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[Embedding dimension $d = 5$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/uniformsynth_softmax_dim5_100prod.pdf}
}
\subfloat[Embedding dimension\\ $d = 10$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/uniformsynth_softmax_dim10_100prod.pdf}
}
\hfill
\subfloat[Embedding dimension $d = 15$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/uniformsynth_softmax_dim15_100prod.pdf}
}    
\subfloat[Embedding dimension $d = 20$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/uniformsynth_softmax_dim20_100prod.pdf}
}
\caption{Average user weight on each feature (blue) and fraction of producers going for each feature (red) for the softmax serving rule; $n=100$ producers. Uniform distribution of users.\label{fig:uniformsoftmax_n100}}
\end{figure}


\begin{figure}[!h]
\vspace{-2mm}
\centering
\captionsetup[subfigure]{justification=centering}
\subfloat[Embedding dimension\\ $d = 5$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/Movielens_softmax_dim5_100prod.pdf}
}
% \hfill
\subfloat[Embedding dimension\\ $d = 10$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/Movielens_softmax_dim10_100prod.pdf}
}
\hfill
\subfloat[Embedding dimension $d = 15$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/Movielens_softmax_dim15_100prod.pdf}
}
\hfill
\subfloat[Embedding dimension $d = 20$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/Movielens_softmax_dim20_100prod.pdf}
}
\caption{Average user weight on each feature (blue) and fraction of producers going for each feature (red) for the softmax serving rule with $n=100$ producers. User embeddings obtained from NMF on MovieLens-100k.}\label{fig:movielens-100k-softmax}
\end{figure}


In Figure~\ref{fig:skewed_n100_linear}, we consider the case of users generated according to our skewed-uniform  distribution, where features are numbered in increasing order of weight, and of the linear-proportional content-serving rule. Interestingly, we note that the equilibrium does not have producers picking features proportionally to the weight on each feature as per Section~\ref{sec:simple_eq}, and many features are not chosen by the producers at all. This is even though we are using the linear-proportional content-serving rule (and not the softmax of Figure~\ref{fig:uniformsoftmax_n100}, which strongly incentivizes going after the best features) as in Figure~\ref{fig:uniform_n100}, and even though we have little randomness due to the large sample size of $K = 10,000$ in our synthetic experiments (unlike in Figure~\ref{fig:movielens-100k-linear}). However, it is still the case that features that have more representation in the user data have more producers choosing them. We believe this is because, compared to Section~\ref{sec:simple_eq}, more subtle effects start arising. In Section~\ref{sec:simple_eq}, a producer that picked feature $f$ only reached users interested in feature $f$ and only competed with other producers who picked $f$. This gave incentives to producers to target under-represented features if they had little competition for that feature. However, in our experiments, users are not single-minded and have weight in every direction, meaning that a producer investing in feature $f$ is reaching and competing over all users, and in turn against all other producers. This then gives producers incentives to ignore underrepresented features, as this leads producers to be less competitive on a significant fraction of users. Instead, it is better for producers to compete by trying to match their content to the features that are likely to match well and be seen by a large fraction of the consumer base. These features roughly coincide with the features that are most represented in the data. A direct consequence of this lessened competition is less specialization than in the uniform case.


\begin{figure}[!h]
\centering
\vspace{-4mm}
\captionsetup[subfigure]{justification=centering}
\subfloat[Embedding dimension\\ $d = 5$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/WeightedSynth_linear_dim5_100prod.pdf}
}
% \hfill
\subfloat[Embedding dimension\\ $d = 10$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/WeightedSynth_linear_dim10_100prod.pdf}
}
\hfill
\subfloat[Embedding dimension $d = 15$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/WeightedSynth_linear_dim15_100prod.pdf}
}
\hfill
\subfloat[Embedding dimension $d = 20$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/WeightedSynth_linear_dim20_100prod.pdf}
}
\caption{Average user weight on each feature (blue) and fraction of producers going for each feature (red) for the linear-proportional serving rule; $n =100$ producers. Skewed-uniform distribution of users.}\label{fig:skewed_n100_linear}
\end{figure}

\begin{figure}[!h]
\centering
\vspace{-7mm}
\subfloat[Embedding dimension\\ $d = 5$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/WeightedSynth_softmax_dim5_100prod.pdf}
}
% \hfill
\subfloat[Embedding dimension\\ $d = 10$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/WeightedSynth_softmax_dim10_100prod.pdf}
}
\hfill
\subfloat[Embedding dimension \\ $d = 15$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/WeightedSynth_softmax_dim15_100prod.pdf}
}
\hfill
\subfloat[Embedding dimension \\$d = 20$]{
    \includegraphics[width=0.23\textwidth]{Figures/engagement-udpd/WeightedSynth_softmax_dim20_100prod.pdf}
}
\caption{Average user weight on each feature (in blue) and fraction of producers going for each feature (in red) for the softmax content serving rule; $n =100$ producers. Skewed-uniform distribution of users.}\label{fig:skewed_n100_softmax}
\vspace{-1mm}
\end{figure}
In Figure~\ref{fig:skewed_n100_softmax}, we consider our skewed-uniform dataset under the softmax serving rule. Compared to Figure~\ref{fig:skewed_n100_linear}, we see even lesser specialization. This is consistent with our previous observations that the softmax rule rewards the ``best'' features, as opposed to diversifying to reduce competition when it comes to reaching users.










==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> rating-maximization.tex <==
Rating utility is $\E_c [(c^T s_i) p_i(c)]$\\
Ff $p_i(c) = \frac{c^T s_i}{\sum_{j=1}^n c^T s_j}$  then notice
\kri{$\frac{x^2}{x+a}$ is convex, so rating maximization is easy over the probability simplex, it must be achieved on some vertex}

if 
$p_i(c) = \frac{\exp{c^T s_i}}{\sum_{j=1}^n \exp{c^T s_j}}$ then the second derivative of the rating is $\E_c[p_i(c)(1-p_i(c))(2 + c^T s_i(1-2p_i(c)))]$
One sufficient condition for convexity is $\abs{c} < 2$ as then
$(2 + c^T s_i(1-2p_i(c)) > 0$, but it general it may not be convex. 


\begin{lemma}{Strictly convex function maximization over a bounded polyhedron \label{SC poly}}{}
Let $f: \R^d \to \R$ be a strictly convex function, then its maximum over the probability simplex $\Delta_{d-1}$, is only achieved at $1$ vertex i.e $\argmax_{\Delta_{d-1}} f = \{e_j \}$ for a single $j \in [d]$   
\end{lemma}

\begin{proof}
(by contradiction)
Let $z \in \Delta_{d-1}$ be a maximizer where $z = \sum_{i=1}^d \lambda_i e_i$ not a vertex, $\therefore \exists$ atleast two unique indices $\lambda_l>0, \lambda_k >0$; and we have

\begin{align*}
    f(z) = f(\sum_{i=1}^d \lambda_i v_i) < \sum_{i=1}^d \lambda_i f(v_i) \leq f(z)
\end{align*}
the above is a contradiction.
\end{proof}

\begin{corollary}{Form of PNE (if they exist) \label{PNE SC}}{}
If the user utility function is strictly convex, \textbf{and} $(s_1, \ldots s_n)$ is a PNE, then each $s_i$ is a vertex of the probability simplex
\end{corollary}

\subsection{Producer utility as engagement with linear probability serving}
Recall linear probabilty serving is $p_i(c) = \frac{c^T s_i}{\sum_{j=1}^n c^T s_j}$, Each producers utility function is $\E_{c} [ \frac{(c^T s_i)^2}{\sum_{j=1}^n c^T s_j}]$ which is strictly convex. \\
First lets see if all same strategy PNE exist, i.e. let $s = (a,a \ldots a)$ be all same strat pure NE, by \eqref{PNE SC} $a = e_j$\\
$u_i(e_j, s_{-i}) = \E_{c}[\frac{c^T e_j}{n}] = \frac{(\sum_{k=1}^m c_k)^T e_j}{nm}$
\kri{TODO}
